A Hardware Co-design Workflow for Scientific Instruments at the Edge

As spatial and temporal resolutions of scientific instruments improve, the explosion in the volume of data produced is becoming a key challenge. It can be a critical bottleneck for integration between scientific instruments at the edge and high-performance computers/emerging accelerators. Placing data compression or reduction logic close to the data source is a possible approach to solve the bottleneck. However, the realization of such a solution requires the development of custom ASIC designs, which is still challenging in practice and tends to produce one-off implementations unusable beyond the initial intended scope. Therefore, as a feasibility study, we have been investigating a design workflow that allows us to explore algorithmically complex hardware designs and develop reusable hardware libraries for the needs of scientific instruments at the edge. Our vision is to cultivate our hardware development capability for streaming/dataflow hardware components that can be placed close to the data source to enable extreme data-intensive scientific experiments or environmental sensing. Furthermore, reducing data movement is essential to improving computing performance in general. Therefore, our co-design efforts on streaming hardware components can benefit computing applications other than scientific instruments. This vision paper discusses hardware specialization needs in scientific instruments and briefly reviews our progress leveraging the Chisel hardware description language and emerging open-source hardware ecosystems, including a few design examples.

==> tmp/chisel.tex <==


\section{Hardware programming ecosystem and design exploration}

Hardware description languages (HDL)~\cite{golson2016language} such as Verilog, VHDL are used to describe digital circuits. Both Verilog and VHDL are originally developed in early 80s with the intent of digital circuit simulation. These languages are eventually adopted for synthesis and ubiquitously used in both industry and academy. However, as the complexity of hardware design requirements increases, the productivity of those traditional HDLs is becoming a huge concern because their language designs are simply old and lacks power language features found in modern languages. One of the biggest problems is that HDLs lack recursive generation, requiring designers to manually unroll, which also degrades the conciseness of the codes and reusability. A good recursive circuit example is a circuit that converts variable-length data blocks to a fixed size buffer~\cite{Ueno:2017hv}, which is crucial for data compression and internally consists of a large barrel shifter or a 2D array of multiplexers. Systolic Arrays~\cite{kung1978systolic}, which are often used to accelerate matrix multiply computation, are also another good example. To compensate the lack of recursive generating capability, designers tend to end up writing their custom generator codes in C++, Python, etc to generate HDL codes. Since HDLs are designed in 80s and behind modern software paradigms like function programming, it is challenging to develop testbench codes if more flexible software references are needed. Thus we started seeking a productive hardware description language that allows us to describe circuit in a concise manner, express recursive structure, and describe testbench more flexibly. 

% low-level presentation
% System Verilog lacks powerful language features 


Coincidentally, hardware programming model exploration is one of the hot topics in the field of computer architecture~\cite{truong2019golden,hennessynew} recently. As the CMOS scaling is coming to end, hardware specialization is becoming a new trend to sustain the performance gain. Industries even previously known as a software company such as Microsoft, Amazon, Google are actively developing their custom accelerators and processors. This new custom hardware trend is becoming a good tailwind to hardware ecosystem, including open-source instruction-set such as RISC-V~\cite{asanovic2014instruction}, open-source hardware implementations~\cite{celio2017boomv2,fatollahi2014opensoc} and open-source hardware tools~\cite{wolf2013yosys,Bachrach:ft,izraelevitz2017reusability,snyder2013verilator}. Google also recently announced that an open-source foundry PDK~\cite{ansell2020missing}. With the advent of innovative semiconductor companies like efabless.com, even a small group can tape-out a chip with significantly lower cost, benefiting from a fully open-source end-to-end ASIC design flow~\cite{edwards2021real}.


\subsection{Chisel hardware construction language}

Largely inspired by RISC-V agile development approach~\cite{lee2016agile}, we employ an emerging hardware construction language named Chisel~\cite{Bachrach:ft,bachrach2017chisel,schoeberl2020digital} for our compressor circuit design exploration. Chisel is a class library written in Scala that allows us to describe synthesizable digital circuits and simulate them seamlessly. Leveraging the power of modern programming language paradigms, Chisel offers higher expressivity that dramatically improves the productivity of the circuit design process. In fact, Chisel is used for many real-world tapeout designs~\cite{Asanovic:EECS-2016-17,celio2017boomv2,bailey201828nm,cass2019taking} (e.g., RISC-V processors, Google’s Edge TPU) and the Chisel community keeps growing. Chisel is also popular in academic for architecture researches~\cite{di2018parallel,serre2018dsl,nowatzki2017stream,prabhakar2017plasticine}. Several studies confirmed that Chisel significantly reduces the code size, improves the code reusability and incurs no performance penalty (the most cases the exact same frequency) as Verilog~\cite{arcas2014empirical,mosanu2019flexi,kwon2017opensmart}.

Listings \ref{verilog} and \ref{chisel} show a comparison between Verilog and Chisel on a simple counter circuit. This example renders some fundamental features in Chisel, compared to Verilog. First of all, the Chisel version has no clock, reset signals and \lstinline|always| blocks because it automatically infers clock and reset signals when needed. Since the default form of the state element provided by Chisel is a positive-edge register that supports synchronous reset, no \lstinline|always| blocks are needed.
%\lstinline|RegNext()| delays its input by one clock cycle and copies it to the output. 
Such restriction in the state element enforces a design guideline transparently and makes Chisel syntax more concise at the cost of flexibility. Chisel provides frequently-used data types such as Int, UInt, Int, instead of a range of bits like in Verilog, which also improves readability. This Chisel code snippet also includes an example of parameterization; the Counter class accepts the max value of the counter when instantiating and calculates the required bit length for the counter.

\begin{lstlisting}[language=verilog,caption={Simple counter in Verilog},captionpos=b,label={verilog},frame=single]
module Counter(
   input        clock,
   input        reset,
   output [3:0] io_out
);
   reg [3:0]  cntReg;
   assign io_out = cntReg;
   
   always @(posedge clock) begin
   if (reset) begin
        cntReg <= 4'h0;
   end else begin
        if (cntReg == 4'h9) begin
           cntReg <= 4'h0;
        end else begin
           cntReg <= cntReg + 4'h1;
        end
     end
   end
endmodule
\end{lstlisting}

\begin{lstlisting}[language=scala,caption={Simple counter in Chisel},captionpos=b, label={chisel},frame=single]
class Counter(val max:Int = 10) extends Module {
  val nbits = log2Ceil(max+1)
  val io = IO(new Bundle {
    val out = Output(UInt(nbits.W))
  })
  val cntReg = RegInit(0.U(nbits.W))
  cntReg := cntReg + 1.U
 
  when( cntReg === (max-1).U ) {
    cntReg := 0.U
  }
  io.out := cntReg
}
\end{lstlisting}

One of the important aspect of Chisel is that it encourages test-driven development and offers fully integrated testing harnesses so that users can write test-bench codes in Scala. Listing~\ref{testbench} is a simple testbench for the counter circuit (Listing~\ref{chisel}). Testbench codes are also written in Scala. Scala is a powerful general-purpose modern programming language, which means complex data processing can done in a testbench. Testbenches for our compressor components directly read and analyze huge X-ray datasets and feed selected regions to our compressor designs running in a circuit simulator to verify the functionality.
% software/hardware co-design can be done through test-bench development.
Running user testbench codes is straightforward in Chisel and requires no high-end machine. Chisel simulates the behavior of generated circuits using either an internal Scala-based simulator or Verilator~\cite{snyder2013verilator} that translates Verilog codes into C++ codes for faster simulation. We found Chisel's integrated test environment accelerate the iteration of the design loop (coding, compiling, evaluating), which helps our design exploration even though the I/O layout and parameters change during the design exploration.

\begin{lstlisting}[language=Scala, caption={Testbench for counter}, captionpos=b, label={testbench},frame=single]
class CounterUnitTester(c: Counter) extends PeekPokeTester(c) {
  val max = c.max
  for (i <- 0 until max*2) {
    expect(c.io.out, i % max) // verify
    step(1) // advance the clock
  }
}
\end{lstlisting}

\begin{lstlisting}[language=Scala, caption={Metadata generation in Chisel}, captionpos=b, label={bitmask},frame=single]
class BitMask(val n:Int=8, val w:Int=12) extends Module {
  val io = IO(new Bundle {
    val in  = Input(Vec(n, UInt(w.W)))
    val out = Output(UInt(n.W))
  })
  val metadata = VecInit.tabulate(n)
    {i => isnz(io.in(i))<<i}
  io.out := metadata.reduce(_ | _)
}
\end{lstlisting}

Listing \ref{bitmask} is a code snippet that demonstrates constructing circuits using functional programming language syntax. The BitMask module takes a vector of integer values as an input, where the length of vector is $n$ and the bit-width of each integer is $w$, and outputs a bitmask (n-bit integer) whose bits are associated with integers in the input vector. Each bit in the bitmask is set 1 if the content of associated integer is non-zero, otherwise 0. It first iterates over an input vector and generates another vector that element is a separate bit-mask value for associated input at 
\lstinline|VecInit.tabulate()|. A user-defined function \lstinline|isnz()| returns 1 if \lstinline|io.in(i)| is non-zero, otherwise 0. Then, \lstinline|metadata| is reduced with the OR operation into an integer (bitmask) at \lstinline|reduce()|.

Another powerful capability of Chisel is that its ability of constructing recursive hardware structure in a software-like manner. Many hardware algorithms can be described as a dividend and conquer algorithm, including the previously-mentioned reduction stage in our on-chip compressor. Such circuit can be huge, depending on parameters such as input size. With a 128-row pixel array, the number of lines of the reduction in Verilog can be an order of ten thousands. It is certainly too expensive to maintain such code during design exploration since requirements and constraints often change. Listing \ref{recursive} is a divide and conquer implementation example of leading zero counting. Although it omits details on bit-length calculation, it shows an overall idea of how to construct recursive structure; it divides the problem size half until it reaches to the minimum size.

\begin{lstlisting}[language=Scala, caption={Recursive structure: counting leading zeros}, captionpos=b, label={recursive},frame=single]
class Clz(nb: Int = 16) extends Module {
  val half = nb >> 1
  val lognb = log2Ceil(nb)
  val io = IO(new Bundle {
    val in = Input(UInt(nb.W))
    val out = Output(UInt((lognb+1).W))
  })
  // Clz2() is for the size two.
  val c0 = if (half==2) Module(new Clz2()) else Module(new Clz(half))
  val c1 = if (half==2) Module(new Clz2()) else Module(new Clz(half))
  c0.io.in := io.in(half-1, 0)
  c1.io.in := io.in(nb-1, half)
  io.out := // merge c1 and c0
}
\end{lstlisting}

%\begin{lstlisting}[language=Scala, caption={
%scala> val a  = Vector.tabulate(4) {i => 1<<i}
%Vector(1, 2, 4, 8)
%scala> a.reduce(_ | _)
%15
%\end{lstlisting}

% Scala snippets
% pros & cons: particularly cons. mixed data type with Scala. 
% generalization, ability to express algorithm, instead of implementation
% powerful features, vector type, utility libraries,  recursive instantiation, test-driven development. lack: pipeline manual
% summary of Chisel with examples. explain Data type, recursive structure, etc

\subsection{Practical viewpoint}

%We summarize Chisel from a practical viewpoint, based on our experiences.
Setting up Chisel programming environment is straightforward as long as both Java development environment and an interactive build tool named \textit{sbt} are installed\footnote{Java environment is usually installed by default.}.
An abundance of documents/tutorials and open-source codes written in Chisel are available online. Since Chisel itself is also an open-source code, further details can be obtained by browsing its source code if needed. Chisel communities are active and growing, consisting of hardware and software experts. Such trait can be a great benefit over commercial design tools and can attract more developers. As the integration needs of more complicated algorithms such as AI inference to ASIC, Chisel can bridge between hardware and software experts, thanks to its RTL-level abstraction with higher-level language constructs.

Chisel’s higher expressivity, particularly for recursive structures, allows us to focus hardware algorithms of interest, which not only reduces the number of lines of code significantly compared to Verilog, but also allows us to capture design patterns easily and improves the design reusability. Another great benefit is that we write testbenches in Scala, a powerful modern programming language that is used in production environments. In fact, we implement various compression encoding schemes directly in Scala to run software-based simulation and use those software-based encoding schemes to verify the outputs from test circuits that run in a cycle accurate simulator. 

Chisel assumes positive-edge trigger registers and synchronous reset by default, which restricts the flexibility in hardware designs and may be considered this as a disadvantage. However, restricting the behavior of circuits can possibly reduce the cost of validation significantly. Recent versions of Chisel supports asynchronous reset and multiple clock domains. Another possible disadvantage is that Verilog codes generated by Chisel tend not to always be human-readable but Chisel community realized such issue and there are efforts to improve its generator.


% modern language+library help Golden model as a reference or verify 
% resource usage, simulation speed
% the original Chisel paper, etc
% about existing Chisel hardware libraries
